Guaranteed Scalable Learning of Latent Tree Models

We present an integrated approach for structure and parameter estimation in latent tree graphical models. Our overall approach follows a "divide-and-conquer" strategy that learns models over small groups of variables and iteratively merges onto a global solution. The structure learning involves combinatorial operations such as minimum spanning tree construction and local recursive grouping; the parameter learning is based on the method of moments and on tensor decompositions. Our method is guaranteed to correctly recover the unknown tree structure and the model parameters with low sample complexity for the class of linear multivariate latent tree models which includes discrete and Gaussian distributions, and Gaussian mixtures. Our bulk asynchronous parallel algorithm is implemented in parallel and the parallel computation complexity increases only logarithmically with the number of variables and linearly with dimensionality of each variable.

==> 7.5conclusion.tex <==

\section{CONCLUSION}\label{section:Conclusion}

We present an integrated approach to structure and parameter estimation in latent tree models. 
Our method overcomes challenges such as uncertainty of location and number of hidden variables, problem of local optima with no consistency guarantees, difficulty in scalability with respect to number of variables. The proposed algorithm is ideal for parallel computing and highly scalable. %We successfully applied the algorithm to a real application for disease hierarchy discovery using large patient data for 1.6M patients. 
%Please find the appendix \href{https://drive.google.com/file/d/1ZkKVJjLrI1aMf-VevMJT1B1saXhtXcmK/view?usp=sharing}{\underline{here}}. 



%The ``divide-and-conquer'' manner of learning the latent tree graphical model incorporates a local recursive information distance test to learn the structure and a triplet spectral decomposition to learn parameters which are both consistent globally. %In other words, our method  is guaranteed to correctly recover the unknown tree structure and the model parameters with low sample complexity for the class of linear multivariate latent tree models.
%We implement our algorithm in parallel using the OpenMP framework and it scales logarithmically with the number of variables and linearly with dimensionality along each variable. We analyze two large datasets of electronic health records. The results show that our proposed algorithm generates intuitive and clinically meaningful disease hierarchies.\href{https://drive.google.com/file/d/1ZkKVJjLrI1aMf-VevMJT1B1saXhtXcmK/view?usp=sharing}{Appendix}

